First results from the JWST Early Release Science Program Q3D: Turbulent times in the life of a $z \sim 3$ extremely red quasar revealed by NIRSpec IFU

Extremely red quasars, with bolometric luminosities exceeding $10^{47}$ erg s$^{-1}$, are a fascinating high-redshift population that is absent in the local universe. They are the best candidates for supermassive black holes accreting at rates at or above the Eddington limit, and they are associated with the most rapid and powerful outflows of ionized gas known to date. They are also hosted by massive galaxies. Here we present the first integral field unit (IFU) observations of a high-redshift quasar obtained by the Near Infrared Spectrograph (NIRSpec) on board the James Webb Space Telescope (JWST), which targeted SDSSJ165202.64+172852.3, an extremely red quasar at $z=2.94$. JWST observations reveal extended ionized gas - as traced by [OIII]$\lambda$5007\AA - in the host galaxy of the quasar, its outflow, and the circumgalactic medium. The complex morphology and kinematics imply that the quasar resides in a very dense environment with several interacting companion galaxies within projected distances of 10-15 kpc. The high density of the environment and the large velocities of the companion galaxies suggest that this system may represent the core of a forming cluster of galaxies. The system is a good candidate for a merger of two or more dark matter halos, each with a mass of a few $10^{13}$ M$_\odot$ and traces potentially one of the densest knots at $z\sim3$.

==> addons.tex <==
Indeed, there are now observations of a handful of other sources sharing these two properties -- very high velocity dispersion and a large number of nearby companions -- with J1652.  For example, the environment of the powerful radio-loud AGN PKS 1138-262 at $z \sim 2.2$, called the Spiderweb Galaxy, is located in a massive galaxy with $\sim 10^{12}$~M$_{\odot}$ \citep{Seymour_2007, Hatch_2009} and its environment is the prime example of a forming galaxy cluster. Deep \hst\ imaging shows tens of satellite galaxies \citep{Miley_2006}, and the rest-frame far-UV continuum morphology of the radio galaxy is clumpy indicative of strong active merging, which has earned it its name ‘Spiderweb galaxy’. Using deep ground-based IFU observations with the Spectrograph for INtegral Field Observations in the Near Infrared \citep[SINFONI,][]{Eisenhauer_2003}, \citet{Kuiper_2011} performed a detailed study of the kinematics of the galaxies within 60 kpc of the radio core and they find that 11 galaxies are at the redshift of the protocluster, implying a galaxy overdensity in the core of $\sim$ 200. Quite intriguing is also the even smaller-scale environment around the Spiderweb galaxy. \citet{Kuiper_2011} confirms at least three companion galaxies within 20~kpc of the Spiderweb galaxy with velocity offsets of $400-1100$~km/s and narrow emission lines ([OII] and \oiii\ emission with $\sigma < 300$~km/s). The galaxy velocity dispersion of the cluster galaxies in the central $120 \times 120$~kpc$^{2}$ of the protocluster is broad and double-peaked with a velocity dispersion of $1360 \pm 206$~km/s. Taking into account the observed properties of the core as well as the larger-scale environment, the most likely scenario in comparison with simulations \citep{Springel_2006, Delucia_2007} is that the Spiderweb protocluster consists of two galaxy groups with dark matter halo masses of several $\times 10^{13}$~M$_{\odot}$ each that are in the process of merging. 

With respect to the density of the immediate 15-20~kpc environment, similar observations have been made in the cores of other high-z galaxy clusters, for example a cluster at $z = 4.3$ in the field of the sub-mm source SPT2349-56 \citep{Miller_2018}. Using deep ALMA spectral imaging, multiple cluster members are confirmed to be within 15~kpc with velocity offsets of up to 700~km/s. This cluster is different from the Spiderweb cluster in that the observed kinematics and spatial configuration of the galaxies suggest that the structure more likely represents a single gravitationally bound halo rather than multiple groups. The velocity dispersion of $\sim 410$~km/s of the galaxies and other arguments suggest that this system represents the core of a cluster of galaxies that is at an advanced stage of formation at $z = 4.3$.

While observations that would allow conclusions about the large-scale environment around J1652 are not available, the present NIRSpec observations in concert with the \hst\ imaging and the fact that the host of J1652 is very massive ($\log{M_*/M_{\odot} \sim 11.4-12.4}$) indicate that the 20~kpc-scale environment of J1652 is similar in terms of galaxy density and kinematics to what is observed in some of the densest knots in the high-redshift Universe and predicted in simulations \citep{Behroozi_2013, Wu_2013}. While it is difficult to predict the halo masses that such a structure would evolve into by $z=0$ owing to the large halo-to-halo variations in dark-matter halo-growth histories (reference), the observations suggest that the J1652 environment could well be hosted by a dark matter halo of $\sim 10^{14}$~M$_{\odot}$ and could be the progenitor of a galaxy cluster halo with $M > 10^{15}$~M$_{\odot}$ at $z=0$.


